AnyTask: an Automated Task and Data Generation Framework for Advancing Sim-to-Real Policy Learning

Generalist robot learning remains constrained by data: large-scale, diverse, and high-quality interaction data are expensive to collect in the real world. While simulation has become a promising way for scaling up data collection, the related tasks, including simulation task design, task-aware scene generation, expert demonstration synthesis, and sim-to-real transfer, still demand substantial human effort. We present AnyTask, an automated framework that pairs massively parallel GPU simulation with foundation models to design diverse manipulation tasks and synthesize robot data. We introduce three AnyTask agents for generating expert demonstrations aiming to solve as many tasks as possible: 1) ViPR, a novel task and motion planning agent with VLM-in-the-loop Parallel Refinement; 2) ViPR-Eureka, a reinforcement learning agent with generated dense rewards and LLM-guided contact sampling; 3) ViPR-RL, a hybrid planning and learning approach that jointly produces high-quality demonstrations with only sparse rewards. We train behavior cloning policies on generated data, validate them in simulation, and deploy them directly on real robot hardware. The policies generalize to novel object poses, achieving 44% average success across a suite of real-world pick-and-place, drawer opening, contact-rich pushing, and long-horizon manipulation tasks. Our project website is at https://anytask.rai-inst.com .

==> figures_and_tables/data_collection_success.tex <==
\begin{table}[H]
    \centering
    \caption{Data collection speed for different methods on lifting task. Rendering time are for 4 rgbd cameras per scene, point cloud computations, and chucked saving}
    \begin{tabular}{lccc}
    \toprule
     & ViPR & ViPR-RL & Vi \\
     Collection Time & 28.9& & \\
     Rendering Time& &34.6 & \\
     Total Time &  & 63.5& \\
    \bottomrule
    \end{tabular}
    \label{tab:bleu_score}
\end{table}

==> figures_and_tables/data_generation_speed.tex <==
\begin{table*}[tbh]
    \centering
    \caption{Data generation speed.}
    % \resizebox{\columnwidth}{!}{
    \resizebox{\linewidth}{!}{
    \begin{tabular}{|c|cccccc|}
    \hline
      & Real world teleop & GenSim2~\cite{huagensim2} & Simulated teleop & Ours (scripted) & Ours (RL) & Ours (scripted + RL)   \\
     \hline
     \hline
     Compute time per task & - & & & & & \\
     Human time per task & & & & & &\\
     \hline
     Compute time per demo & - & & & & & \\
     Human time per demo & & & & 0 & 0 & 0\\
     

     
     
     \hline
    \end{tabular}
    }
    \label{tab:data_generation_speed}

    
\end{table*}

==> figures_and_tables/human_evaluated_success_checker.tex <==
\begin{table}[H]
    \centering
    \caption{Human Evaluation of Success Checkers}

    \resizebox{0.9\linewidth}{!}{ %
    \begin{tabular}{ccccc}
    \toprule
        Lifting  & Pushing  & Stacking & Pick \& Place & Drawer opening \\
      80 \% & 100 \% & 100 \%  & 100 \% & 100 \% \\ 
    \bottomrule
    \end{tabular}
    \label{tab:human_eval}%
    }
\end{table}
